Massively Parallel and Dynamic Algorithms for Minimum Size Clustering

In this paper, we study the $r$-gather problem, a natural formulation of minimum-size clustering in metric spaces. The goal of $r$-gather is to partition $n$ points into clusters such that each cluster has size at least $r$, and the maximum radius of the clusters is minimized. This additional constraint completely changes the algorithmic nature of the problem, and many clustering techniques fail. Also previous dynamic and parallel algorithms do not achieve desirable complexity. We propose algorithms both in the Massively Parallel Computation (MPC) model and in the dynamic setting. Our MPC algorithm handles input points from the Euclidean space $\mathbb{R}^d$. It computes an $O(1)$-approximate solution of $r$-gather in $O(\log^{\varepsilon} n)$ rounds using total space $O(n^{1+\gamma}\cdot d)$ for arbitrarily small constants $\varepsilon,\gamma > 0$. In addition our algorithm is fully scalable, i.e., there is no lower bound on the memory per machine. Our dynamic algorithm maintains an $O(1)$-approximate $r$-gather solution under insertions/deletions of points in a metric space with doubling dimension $d$. The update time is $r \cdot 2^{O(d)}\cdot \log^{O(1)}\Delta$ and the query time is $2^{O(d)}\cdot \log^{O(1)}\Delta$, where $\Delta$ is the ratio between the largest and the smallest distance.

==> useless.tex <==
Let the input point set be $P=\{p_1,p_2,\cdots,p_n\}\subset \mathbb{R}^d$. 
The goal of $r$-gather is to partition $P$ into several subsets $P_1,P_2,\cdots,P_t$ and assign each subset $P_i$ a center $c_i\in P_i$ such that $\forall i\in [t], |P_i|\geq r$ and $\max_{i \in [r]}\max_{p\in P_i} \dist(c_i,p)$ is minimized.
Let the optimal radius be $\rho^*(P)$. 
If $P$ is clear in the context, we use $\rho^*$ to denote $\rho^*(P)$ for short.


For a point $p\in P$, let $\rho_r(p)$ denote the distance between $p$ and the $r$-th closest neighbor $q\in P$.
Let $\hat{\rho} = \max_{p\in P} \rho_r(p)$. 

\begin{lemma}
$\rho^*\geq \hat{\rho}/2$.
\end{lemma}
\begin{proof}
Let $P_1,P_2,\cdots, P_t$ be the optimal partition of $P$ and let $c_1,c_2,\cdots, c_t$ be the corresponding centers.

Consider a point $p\in P$. 
Let $P_i$ be the subset containing $p$.
Let $q$ be a point in $P_i$ which is the farthest point from $p$.
We have $\rho^*\geq \max(\dist(p,c_i),\dist(q,c_i))\geq \dist(p,q)/2\geq \rho_r(p)/2$ where the last inequality follows from that $P_i$ contains at least $r$ points and $q$ is the point farthest from $p$ in $P_i$.
\end{proof}


We show an offline algorithm as the following:
\begin{enumerate}
    \item Construct a graph $G=(P,E)$ where each vertex corresponds to a point $p\in P$.
    The number of edges $|E|\leq O(n\cdot r)$. 
    For each vertex $p$, it has at least $r$ neighbors in $G$. 
    Each edge $(p,p')\in E$ satifies $\dist(p,p')\leq c\cdot \hat{\rho}$ where $c\geq 1$ is some constant.
    \item Find an arbitrary maximal subset of vertices $S\subseteq P$ such that $\forall p,p'\in S$, $\dist_G(p,p')\geq 3$. 
    In other words, $S$ is a maximal independent set in $G^2$.
    \item Partition $P$ into $|S|$ subsets where each point in $S$ is a center of a subset.
    For each point $p\in P\setminus S$, assign $p$ to a subset with center $c\in S$ such that $\dist_G(p,c)$ is minimized.
\end{enumerate}

\begin{lemma}
Let $P_1,P_2,\cdots,P_t$ be the partition obtained by the above procedure.
Let $c_1,c_2,\cdots,c_t$ be the centers of $P_1,P_2,\cdots,P_t$ respectively.
We have $\forall i\in[t], |P_i|\geq r$ and $\forall p\in P_i,\dist(p,c_i)\leq 2\cdot c\cdot \hat{\rho}$.
\end{lemma}
\begin{proof}
By our construction, since $S$ is a maximal independent set in $G^2$, we have $\forall i\in[t],p\in P_i$, $\dist_G(p,c_i)\leq 2$.
Since each edge $(p,p')\in E$ satisfies $\dist(p,p')\leq c\cdot \hat{\rho}$, we have $\forall i\in[t],p\in P_i,$ $\dist(p,c_i)\leq 2\cdot c\cdot \hat{\rho}$.


Consider a subset $P_i$ with center $p\in S$.
Since $\forall q \neq p \in S$, $\dist_G(p,q)\geq 3$, any point $p'$ with $\dist_G(p',p)\leq 1$ must be assigned to the subset $P_i$.
Since the degree of each vertex in $G$ is at least $r$, the size of $P_i$ is at least $r$. 
\end{proof}

We assume the minimum distance between points in $P$ is $1$, and the maximum distance is at most $\Delta$.

To construct graph $G$, we run $\log\Delta$ parallel copies of the following procedure and each copy corresponds to a different parameter $\delta\in \{1,2,4,8,\cdots, \Delta\}$:
\begin{enumerate}
\item Draw $s=\tilde{\Theta}\left(n^{O(1/c^2)}\right)$ different independent LSH functions $h_1,h_2,\cdots,h_s$ with parameter $\delta$ and $c$.
\item $\forall i\in [s],\forall p\in P$, compute $h_i(p)$.
\item $\forall i\in [s], \forall p\in P$, connect $p$ to $r$ arbitrary points $q$ in $G$ with $h_i(p)=h_i(q)$. 
If there are less than $r$ points with $h_i(q)=h_i(p)$, connect $p$ to all such $q$ in $G$.
\item Remove duplicated edges.
\item If there exists a point $p$ which has degree less than $r$, output FAIL.
\item Otherwise, output $G$.
\end{enumerate}
We keep the graph $G$ with the smallest $\delta$ such that the above procedure does not output FAIL.

\begin{lemma}
For the procedure to construct $G$,
the total space needed is $\tilde{O}(n^{1+O(1/c^2)}\cdot r)$ and the number of rounds is $O(1)$.
Furthermore, the obtained graph $G=(P,E)$ satisfies that $\forall p\in P$, the degree of $p$ in $G$ is at least $r$ and with probability at least $0.99$, $\forall (p,p')\in E$, $\dist(p,p')\leq 2\cdot c\cdot \hat{\rho}$. 
\end{lemma}
\begin{proof}
(Omitted.)
\end{proof}

Once we obtain $G$, we need to run maximal independent set on $G^2$. %{\color{red}Peilin: Need to improve this part.}

Finally, we need to run BFS using $2$ rounds to assign points to corresponding subsets.

We can run parallel greedy algorithm for $G^2$. 
We do not need to build $G^2$ explicitly.
The algorithm is shown as the following:
\begin{enumerate}
    \item Permute the labels of vertices randomly. 
    \item Initialize the final solution $S\gets\emptyset$.
    Let $l(p)$ denote the label of $p$.
    \item Repeat until $G$ is empty: \label{it:MIS_major_loop}
    \begin{enumerate}
        \item For each vertex $p$ in $G$, initialize $h(p):=l(p)$.
        \item Repeat $2$ rounds:
        \begin{enumerate}
            \item Simultaneously check each vertex $p$ in $G$: if a neighbor $p'$ of $p$ has $h(p')<h(p)$, update $h(p):=h(p')$.
        \end{enumerate}
        \item Mark each vertex $p$ with $h(p)=l(p)$ as \emph{inactive} and add $p$ to $S$.
        \item Repeat $2$ rounds:
        \begin{enumerate}
            \item Simultaneously check each vertex $p$ in $G$: if a neighbor $p'$ of $p$ is marked as inactive, mark $p$ as inactive.
        \end{enumerate}
        \item Remove all vertices from $G$ that are marked as in active. 
    \end{enumerate}
\end{enumerate}

\begin{lemma}[\cite{?}]
With high probability, the step~\ref{it:MIS_major_loop} will repeat at most $O(\log n)$ rounds.
\end{lemma}

\subsection{$r$-Gather with Outliers}
In the setting that point set $P$ has at most $k$ outliers, the goal is to find a subset $S$ with $|S|\leq k$ such that $\rho^*(P\setminus S)$ is minimized.

Consider an arbitrary $R\geq 2 \cdot \min_{S\subseteq P:|S|\leq k}\rho^*(P\setminus S)$.
Construct the graph $G_R=(P,E)$ as the following: 
for each vertex $p\in P$, we connect $p'$ to $p$ for every $p'$ with $\dist(p,p')\leq R$.

\begin{lemma}
The size of $r$-core of $G_R$ is at least $n-k$.
\end{lemma}
\begin{proof}
Let $S\subseteq P$ satisfies $|S|\leq k$ and $2\cdot \rho^*(P\setminus S)\leq R$.
Let $P_1,P_2,\cdots,P_t$ be the optimal partition of $P\setminus S$. 
Consider an arbitrary vertex $p\in P\setminus S$.
If $p$ is from the cluster $P_i$, then $\dist(p,p')\leq 2\cdot\rho^*(P\setminus S)\leq R$ for every $p'\in P_i$.
Since $|P_i|\geq r$ for $i\in[t]$, we can conclude that $P\setminus S$ is a subset of $r$-core of $G_R$.
\end{proof}

Then we can run MIS on the squared graph of $r$-core of $G_R$ to find clusters such that each cluster has size at least $r$ and the radius of each cluster is at most $2R$.

\subsection{A Stronger Variant of $r$-Gather}
In addition to the original requirement of $r$-gather, we also requires the centers of the partitions satisfies the following property: if $p$ is in the subset $P_i$, then the distance between $p$ and the corresponding center $c_i$ is at most $C\cdot \rho_r(p)$ where $C\geq 1$ is a universal constant.

To achieve this goal, we run the following algorithm:

\begin{enumerate}
    \item Let $t\gets 0$. Initialize the family of partitioned subsets: $\mathcal{P}\gets \emptyset$
    \item Enumerate $R=1, 2, 4, 8,\cdots, \Delta$:
    \begin{enumerate}
        \item Construct the graph $G_R=(P,E)$ as the following: for each vertex $p\in P$, we connect $p'$ to $p$ for every $p'$ with $\dist(p,p')\leq R$.
        \item Compute the $r$-core of $G_R$. Let $G'_R$ be the subgraph of $G_R$ induced by the $r$-core.
        \item For each vertex $p$ in $G'_R$, if it is already in the partition $\bigcup_{P\in\mathcal{P}} P$, delete $p$ and its neighbors from $G'_R$ and let $G''_R$ be the resulting graph.
        \item Compute MIS $S$ of ${G''_R}^2$.
        \item For each $p$ in $S$, create a partition $P$
    \end{enumerate}
\end{enumerate}
